PathoArgus: Advancing Evidence-Grounded Long-Context Visual Reasoning across Gigapixel Whole-Slide and Multi-Slide Case Contexts

Whole-slide pathology reasoning requires models to integrate gigapixel-scale visual evidence across complete case-linked slides, yet current question-answering benchmarks primarily measure final answer accuracy--a metric vulnerable to linguistic priors and benchmark regularities, and insufficient to establish that predictions are grounded in the supplied tissue. We introduce PathoArgus-Bench, a benchmark and evaluation protocol that explicitly tests the full evidence chain: availability, accessibility, use, and responsiveness. PathoArgus-Bench comprises 22,078 four-choice questions from 4,913 patients across 15 TCGA projects, covering six pathology capabilities across three levels of evidence demand, and operates under a fixed reader budget that retains only a small fraction of the gigapixel context. To further isolate evidence-grounded reasoning, we contribute ESG (Evidence State Quartets), a controlled set of 483 quartets where the question text is fixed while the target WSI set is moved, replaced, or removed, requiring consistent predictions across all states. Evaluating 20 general-purpose, medical, and pathology-specific systems reveals a stark gap: while GPT-5.6 achieves 57.09% overall accuracy and 57.04% on ESG, it correctly completes only 19 of 483 quartets (3.93% QExact), exposing that row-level accuracy does not translate into reliable evidence grounding. We also introduce PathoArgus, a fixed-budget reader that allocates context via question relevance and spatial coverage, attaining 50.39% overall accuracy yet only 1.86% QExact--demonstrating that improved context access alone does not ensure consistent evidence-based prediction. Our benchmark and diagnostics establish that acquiring useful whole-slide context is necessary but far from sufficient, and call for a shift from answer-centric to evidence-grounded evaluation in computational pathology.

==> figures/benchmark_profile.tex <==
% Project coverage and context workload are composed with the capability
% hierarchy in figures/capability_hierarchy.tex.


==> figures/construction_pipeline.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[
  font=\sffamily\scriptsize,
  node distance=0.28cm,
  stage/.style={draw=pathblue, rounded corners=2pt, fill=pathlight,
    minimum width=2.25cm, minimum height=0.82cm, align=center},
  gate/.style={draw=pathgreen, diamond, aspect=2.0, fill=pathgreen!9,
    inner sep=1.5pt, align=center},
  pending/.style={draw=pathred, rounded corners=2pt, fill=pathred!8,
    minimum width=2.55cm, minimum height=0.82cm, align=center},
  flow/.style={-{Latex[length=1.8mm]},thick,pathblue}
]
\node[stage] (source) {Source registry\\4,962 patients / 5,516 WSIs};
\node[stage,right=of source] (parse) {Report parsing\\candidate semantic fields};
\node[stage,right=of parse] (qa) {Reverse synthesis\\T1--T5 four-choice QA};
\node[stage,right=of qa] (t6) {Controlled injection\\T6 quartets};
\draw[flow] (source) -- (parse);
\draw[flow] (parse) -- (qa);
\draw[flow] (qa) -- (t6);

\node[gate,below=0.45cm of qa] (format) {format, uniqueness,\\A--D balance};
\draw[flow] (qa) -- (format);

\node[stage,below=1.20cm of source] (split) {Patient split\\70/10/20 stratified};
\node[gate,right=of split] (isolate) {patient/WSI\\overlap = 0};
\node[stage,right=of isolate] (blind) {Blind projection\\remove private metadata};
\node[pending,right=of blind] (expert) {Expert visual review\\\textbf{pending: 0/4,281 gold}};
\draw[flow] (t6.south) |- (split.east);
\draw[flow] (split) -- (isolate);
\draw[flow] (isolate) -- (blind);
\draw[flow] (blind) -- (expert);

\node[align=center,font=\sffamily\scriptsize\bfseries,pathblue]
  at ($(split.south)!0.5!(expert.south)+(0,-0.38)$)
  {22,078 candidate rows $\rightarrow$ 4,281-row blind benchmark split};
\end{tikzpicture}
\caption{Construction pipeline. T1--T5 use reverse synthesis from report fields;
T6 uses controlled movement or removal of a real target WSI set. Automated gates
are complete, but blinded expert visual validation remains the blocking release
stage.}
\label{fig:construction}
\end{figure}


==> figures/running_example.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}[
    font=\sffamily\scriptsize,
    pack/.style={draw=pathblue, rounded corners=1.5pt, minimum width=2.25cm,
      minimum height=0.68cm, align=center, fill=pathlight},
    target/.style={draw=pathred, very thick},
    pred/.style={minimum width=2.25cm, minimum height=0.42cm, align=center},
    label/.style={align=right, font=\sffamily\scriptsize\bfseries}
]
\node[align=center,font=\sffamily\small\bfseries] (q) at (5.25,0.65)
  {Fixed question: Which candidate WSI set contains target-relevant H\&E tissue?};

\node[label] at (-0.35,-0.10) {Visual condition};
\node[pack] (abs) at (1.5,-0.10) {Target absent};
\node[pack] (s1) at (4.0,-0.10) {\textbf{Set 1: target}\\Set 2/3: donors};
\node[pack] (s2) at (6.5,-0.10) {Set 1/3: donors\\\textbf{Set 2: target}};
\node[pack] (s3) at (9.0,-0.10) {Set 1/2: donors\\\textbf{Set 3: target}};
\draw[target] (s1.south west) rectangle (s1.north east);
\draw[target] (s2.south west) rectangle (s2.north east);
\draw[target] (s3.south west) rectangle (s3.north east);

\node[label] at (-0.35,-1.00) {Correct answer};
\node[pred,fill=pathgreen!12] at (1.5,-1.00) {None};
\node[pred,fill=pathgreen!12] at (4.0,-1.00) {Set 1};
\node[pred,fill=pathgreen!12] at (6.5,-1.00) {Set 2};
\node[pred,fill=pathgreen!12] at (9.0,-1.00) {Set 3};

\node[label] at (-0.35,-1.62) {Uniform / FreqPath};
\node[pred,fill=pathred!10] at (1.5,-1.62) {Set 2};
\node[pred,fill=pathred!10] at (4.0,-1.62) {Set 2};
\node[pred,fill=pathred!10] at (6.5,-1.62) {Set 2};
\node[pred,fill=pathred!10] at (9.0,-1.62) {Set 2};

\node[label] at (-0.35,-2.18) {HistoSelect};
\node[pred,fill=pathgold!14] at (1.5,-2.18) {Set 1};
\node[pred,fill=pathgold!14] at (4.0,-2.18) {Set 1};
\node[pred,fill=pathgold!14] at (6.5,-2.18) {Set 1};
\node[pred,fill=pathgold!14] at (9.0,-2.18) {Set 1};

\draw[-{Latex[length=2mm]},pathblue,thick] (abs.north) -- ++(0,0.25);
\draw[-{Latex[length=2mm]},pathblue,thick] (s1.north) -- ++(0,0.25);
\draw[-{Latex[length=2mm]},pathblue,thick] (s2.north) -- ++(0,0.25);
\draw[-{Latex[length=2mm]},pathblue,thick] (s3.north) -- ++(0,0.25);
\node[align=center,text=pathred,font=\sffamily\scriptsize\bfseries]
  at (5.25,-2.75) {Fixed predictions ignore the controlled movement of visual evidence};
\end{tikzpicture}
\caption{Running T6 example. The text remains fixed while the target kidney
case moves among three real candidate WSI sets or is absent. A responsive model
must produce four different decisions. All three current systems repeat a fixed
set identity, yielding 0 quartet exact accuracy for this group. Candidate labels
await pathologist confirmation.}
\label{fig:running-example}
\end{figure}



==> tables/context_allocation_results.tex <==
\begin{table}[t]
\centering
\small
\caption{Fixed-budget context allocation at $K=512$ (\%). \pathoargus leads
Overall and ESG, while Uniform leads Task Macro and all five single-set
capabilities. Systems share CONCH features, the Qwen2.5-7B reader family, and
the final budget, but retain their respective training configurations.}
\label{tab:context-allocation-results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrr}
\toprule
System & Overall$\uparrow$ & Macro$\uparrow$ & GR$\uparrow$ & MA$\uparrow$ & FGR$\uparrow$
& RR$\uparrow$ & CSI$\uparrow$ & ESG$\uparrow$ & QExact$\uparrow$ \\
\midrule
Uniform-K512 & \underline{47.28} & \textbf{52.23} & \textbf{77.99} & \textbf{46.39} & \textbf{42.95} & \textbf{66.59} & \textbf{53.06} & \underline{26.40} & 0.00 \\
HistoSelect-K512~\citep{huang2026histoselect} & 43.28 & \underline{47.65} & 63.56 & \underline{44.29} & \underline{41.61} & \underline{64.76} & \underline{46.26} & 25.41 & 0.00 \\
\textbf{PathoArgus} & \textbf{50.39} & 47.35 & \underline{72.89} & 36.36 & 32.89 & 49.51 & \underline{46.26} & \textbf{46.17} & \textbf{1.86} \\
\bottomrule
\end{tabular}}
\end{table}

